Exploring the Design Space of Static and Incremental Graph Connectivity Algorithms on GPUs

Connected components and spanning forest are fundamental graph algorithms due to their use in many important applications, such as graph clustering and image segmentation. GPUs are an ideal platform for graph algorithms due to their high peak performance and memory bandwidth. While there exist several GPU connectivity algorithms in the literature, many design choices have not yet been explored. In this paper, we explore various design choices in GPU connectivity algorithms, including sampling, linking, and tree compression, for both the static as well as the incremental setting. Our various design choices lead to over 300 new GPU implementations of connectivity, many of which outperform state-of-the-art. We present an experimental evaluation, and show that we achieve an average speedup of 2.47x speedup over existing static algorithms. In the incremental setting, we achieve a throughput of up to 48.23 billion edges per second. Compared to state-of-the-art CPU implementations on a 72-core machine, we achieve a speedup of 8.26--14.51x for static connectivity and 1.85--13.36x for incremental connectivity using a Tesla V100 GPU.

==> framework.tex <==
\section{Framework}\label{sec:framework}

\cw{overall structure}
\cw{how to implement SCC, sp\_tree, DCC here}
\cw{explain EB strategy.}

{\color{red} implementing.}

%%%% BFS
%%%% overall structure
%%%% sampling strategy



%%%% EXPLAINING FRAMEWORK??
%%%% Effect of tiling? (edge ordering)


\changwan{bit-vector BFS}

\begin{comment}

\myparagraph{GPU Implementation Details}
%\changwan{GPU-specific optimizations (load balancing)}
GPUs provide higher peak performance and memory bandwidth than CPUs;
however, evenly distributing edges to process across the massive number of
threads on GPUs is non-trivial.
%Nevertheless, achieving high performance for connected components and spanning forest on GPUs is not trivial due to
%an irregular nature of graphs (different degrees of vertices).
%On GPUs, worklists should be evenly distributed to massive thread.
%Otherwise, resources on GPUs can be poorly utilized, which can significantly degrade performance.
With the \defn{COO} format, threads can process edges in a cyclic
fashion, which is relatively load-balanced \julian{check if true}.
However, when the \defn{CSR} format is used, if each thread is
responsible for processing all of the edges of a vertex, most threads
can be idle if the degrees of vertices are highly skewed (e.g., in
power-law graphs), which can lead to performance degradation due to
poor load-balancing.  Thus, different load-balancing strategies have
been proposed, mainly following into two classes: binary
searching~\cite{Wang2017,DavidsonBGO14,Meng2019} (by which the index
of a source vertex is recovered when edges are processed by threads in
a cyclic fashion \julian{i don't follow this description about binary
searches}), and binning~\cite{Wang2017,Merrill2012,Pai2016,Meng2019},
where vertices with similar degrees are grouped together into a bin,
and then different execution strategies are used for each bin.  In our
implementation, we used a variation of the binning strategy, which we
found to work best in our experiments. In contrast to prior binning
methods which precompute the bins, we use on-the-fly binning, where
only a small number of vertices are partitioned into several bins such
that all bins can reside in the GPU's shared memory (scratchpad
memory).  \julian{i don't follow the binning approach. which are the small number of vertices being partitioned? what does it mean that the bins fit in shared memory? is it the pointers to the bins, or all of the contents of the bins?}
By doing so, we reduce the overhead for creating bins. We
show the effectiveness of our load-balancing strategy in
Section~\ref{sec:eval}.

%% Due to
%% space constraints, we will not show detailed analyses, but we figured
%% out the overhead for binary searches cannot paid off for better load
%% balancing.
%Due to space constraints, we will not show detailed analyses that will be included in the full version of the paper.
%, but we figured out the overhead for binary searches cannot paid off for better load balancing.
%% In addition, in bucketing strategy the buckets are first created and
%% then each bucket is processed in a different way, which can incur a
%% big overhead.  Hence, we adopted a variation of bucketing strategy,
%% and instead of generating buckets in advance, we applied on-the-fly
%% bucketing; only a small amount of vertices are paritioned into several
%% buckets such that all buckets can reside in shared-memory (scratchpad
%% on GPUs).  By doing so, we could reduce the overehad for creating
%% buckets and will show the effectiveness of our load-balancing strategy
%% in Section~\ref{sec:eval}.

%Again, we do not show the effectiveness of our load-balancing strategy here, but by implementing different load-balancing strategies in independent run-time libraries,
%we could see the effectiveness of our strategy.
%\changwan{Some sentences (like we do not show results here) are vulnerable. Emphasizing our load-balancing strategy without evidence may be bad. Should I write this part in a little vague way? Or show experimental results?}

\end{comment}


\begin{comment}

** Add different load-balancing staretgy
exceptions? (
\end{comment}

